Oakestra white paper: An Orchestrator for Edge Computing

Edge computing seeks to enable applications with strict latency requirements by utilizing compute resources deployed closer to the users. The diverse, dynamic, and constrained nature of edge infrastructures necessitates a flexible orchestration framework that dynamically supports application QoS requirements. However, existing state-of-the-art orchestration platforms were designed for datacenter environments and make strict assumptions about underlying infrastructures that do not hold for edge computing. This work proposes a novel hierarchical orchestration framework specifically designed for supporting service operation over edge infrastructures. Through its novel federated cluster management, delegated task scheduling, and semantic overlay networking, our system can flexibly consolidate multiple infrastructure operators and absorb dynamic variations at the edge. We comprehensively evaluate our proof-of-concept implementation -- Oakestra -- against state-of-the-art solutions in both controlled and realistic testbeds and demonstrate the significant benefits of our approach as we achieve approximately 10x and 30% reduction in CPU and memory consumption, respectively.

==> sections/bio.tex <==
\begin{IEEEbiographynophoto}{Giovanni Bartolomeo}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Mehdi Yosofie}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Simon Bäurle}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Oliver Haluszczynski}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Nitinder Mohan}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jörg Ott}
Biography text here.
\end{IEEEbiographynophoto}


==> sections/conclusion.tex <==
\section*{Conclusion}

Here we conclude the paper.

==> sections/edgeio-benefits.tex <==
\section{EdgeIO Design Benefits}
\label{section:benefits}

\textbf{Responsible:
Nitinder + Giovanni + Mehdi
}

% Design Benefits of EdgeIO:
% 1. service scheduling + how it adapts to changes (scale up/down)
% 2. Networking - communication channel
% 3. Decoupled applications development and core EdgeIO workings + supporty for heterogeniety in EgdeIO

\subsubsection{Virtualization}
The possibility to deploy a service using different virtualization technologies, and letting them interact together seamlessly, makes it possible to deploy different applications, use cases, and provides flexibility for developers. 
%
Due to the heterogeneity of edge infrastructures, this characteristic of \sys enables also almost any device to be used as a compute node for a cluster.

%Each service instance, deployed within one of the supported virtualisation technology, is plugged into the network by the Environment Manager with a Veth pair between the custom bridge component and the namespace used for the virtualisation. This means that, for instance, a Docker container, can interact with an Unikernel service deployed on any other node using the same ServiceIP and/or mDNS mechanism. 

\subsubsection{Flexible Networking}

%A typical edge property is that worker nodes reside behind NATs and Firewalls and usually don't have any public IP address. These devices are mostly unreachable outside their network boundaries.
Thanks to the initial polling connection handshake mechanism, \sys can register new workers even in a complex network environment.
Then, compute nodes in different networks do not need an additional VPN or the use of SDN based infrastructures to enable service-to-service communication.
From the application perspective it is possible to dynamically change the routing policy for a network call by just changing a keyword in the hostname of a service or using a different ServiceIP.
%This increases the flexibility for the edge devices and reduces their connectivity restrictions. Security concerns are also solved by design. If no node-to-node communication is needed, operators do not need to open ports on the edge devices. Otherwise, just the tunnel port is enough to guarantee a full communication channel. Is worth noticing that it is still possible to isolate the nodes granting firewall permission only to the well-known clusters through the single tunnel port. This design allows worker nodes to be located behind Firewalls, proxies, NAT-based Routers, and still share their computation capability.
%to function as an orchestration system. In EdgeIO, worker nodes voluntarily share the compute resources to the public cluster manager and poll their tasks from it \circled{7}. This design pattern increases the flexibility in edge environments and makes it possible to combine heterogeneous networks.
%Even applications deployed on a cluster are able to communicate with any of the instances of another service, possibly spread across many other clusters, using the built-in overlay network.

\subsubsection{Microservice-oriented Design}
The internal microservice-oriented design enables replication and high availability of the root and cluster components reducing the possibility of having a single point of failure and making the maintenance and further development easy.

%The message broker does not have to be on the same device as the Cluster Manager, instead, it can be deployed anywhere else, too. The microservice approach within the system and the separation of concerns make maintenance and further development easy

\subsubsection{Scalability and Isolation}
Sending aggregated cluster information to the root orchestrator allows \sys to maintain a high level of separation of context at scale. 
%
At root level, each cluster is seen as a worker node with certain amount of resources. This makes it possible to instantiate dynamically more clusters and to keep the cluster-internal information isolated.
%
At cluster level instead, the nodes are seen like a fleet of heterogeneous compute engines in a heavily async environment. This grants flexibility in the way the workers are managed and enable a high level of horizontal scaling. 

\subsubsection{Compatibility}
How \sys is backwards and horizontally compatible.

\subsection{Fault Tolerance}\label{subsec:faultTol}
A key aspect of the multi-cluster approach of \sys is resiliency. 
%
If an entire cluster fails due to regional outages, other clusters can still operate because clusters are independent of each other.
%
Even nodes can still communicate if they have already resolved the needed routes previously. Services already up and running should not experience disruption.
%
Due to the distributed design, there are various failover alternatives for leader election, task migration, or task rescheduling.

\subsection{Lightweight implementation}
Refer to eval.


